Deep-subwavelength Phase Retarders at Mid-Infrared Frequencies with van der Waals Flakes

Phase retardation is a cornerstone of modern optics, yet, at mid-infrared (mid-IR) frequencies, it remains a major challenge due to the scarcity of simultaneously transparent and birefringent crystals. Most materials resonantly absorb due to lattice vibrations occurring at mid-IR frequencies, and natural birefringence is weak, calling for hundreds of microns to millimeters-thick phase retarders for sufficient polarization rotation. We demonstrate mid-IR phase retardation with flakes of $\alpha$-molybdenum trioxide ($\alpha$-MoO$_3$) that are more than ten times thinner than the operational wavelength, achieving 90 degrees polarization rotation within one micrometer of material. We report conversion ratios above 50% in reflection and transmission mode, and wavelength tunability by several micrometers. Our results showcase that exfoliated flakes of low-dimensional crystals can serve as a platform for mid-IR miniaturized integrated polarization control.

==> tikz/3d-reflection.tex <==
\begin{tikzpicture}
  \node at (0,0) {\includegraphics[width=0.25\linewidth]{data/fig1-3d-reflection.png}};
  \node at (-2,1) {\textbf{(b)}};  
\end{tikzpicture}

==> tikz/3d-transmission.tex <==
\begin{tikzpicture}
  \node at (0,0) {\includegraphics[width=0.25\linewidth]{data/fig1-3d-transmission.png}};
  \node at (-2,1) {\textbf{(b)}};
\end{tikzpicture}

